Toward an Integrated Framework for Automated Development and Optimization of Online Advertising Campaigns

Creating and monitoring competitive and cost-effective pay-per-click advertisement campaigns through the web-search channel is a resource demanding task in terms of expertise and effort. Assisting or even automating the work of an advertising specialist will have an unrivaled commercial value. In this paper we propose a methodology, an architecture, and a fully functional framework for semi- and fully- automated creation, monitoring, and optimization of cost-efficient pay-per-click campaigns with budget constraints. The campaign creation module generates automatically keywords based on the content of the web page to be advertised extended with corresponding ad-texts. These keywords are used to create automatically the campaigns fully equipped with the appropriate values set. The campaigns are uploaded to the auctioneer platform and start running. The optimization module focuses on the learning process from existing campaign statistics and also from applied strategies of previous periods in order to invest optimally in the next period. The objective is to maximize the performance (i.e. clicks, actions) under the current budget constraint. The fully functional prototype is experimentally evaluated on real world Google AdWords campaigns and presents a promising behavior with regards to campaign performance statistics as it outperforms systematically the competing manually maintained campaigns.

==> related.tex <==
\section{Related Work}

%1. GrammAds Related
The research areas of sponsored search, textual advertising and keyword research involve among other topics the automatic extraction, suggestion, and expansion of keywords. An advertising campaign might involve more than one and in most cases a large number of landing pages. The manual selection of even a small set of keywords for advertising purposes is quite laborious, a fact which leads to the recent appearance of commercial tools that create keyword sets directly from a landing page. There exist different techniques for keyword generation. Search engines use query log based mining tools to generate keyword suggestions. In this way, they focus on discovering co-occurrence relationships between terms and suggest similar keywords. They start from an initial key phrase and they are based on past queries that contain these search terms. Google AdWords Keyword Tool \footnote{\url{http://www.adwords.google.com/keywordtool}} exploits this ability and presents frequent queries for the seed set of terms 

Other commercial tools \footnote{\url{http://www.adgooroo.com/}, \url{http://www.wordstream.com/}} determine an advertiser's top competitors and then actively search for the keywords they are targeting. After a period of time, lists of targeted keywords that are competitive for pay per click advertising are automatically generated. These two approaches may result to a recommendation set of keywords which are likely to be general and thus more expensive. Considering this, the challenge of generating keywords is to select both semantically similar and well-focused keywords.

TermsNet and Wordy  \cite{JoshiM06,AbhishekH07} exploit the power of search engines to generate a huge portfolio of terms and to establish the relevance between them. After selecting the most salient terms of the advertiser's web page they query search engines with each initial seed term. With their methods they find other semantically similar terms. Wordy system proposed single word terms (unigrams) for each seed keyword. S. Ravi et al. \cite{RaviBGJPP10} propose a generative model within a machine translation framework so the system translates any given landing page into relevant bid phrases. They first construct a parallel corpus from a given set of bid phrases $b$, aligned to landing page keywords $l$, and then learn the translation model to estimate $Pr(l|b)$ for unseen $(b,l)$ pairs. This approach performs very efficiently but depends on the chosen domain and data that the human decision factor may affect. 

In general, \emph{corpus or domain dependent} systems require a large stack of documents and predetermined keywords to build a prediction model \cite{Liu:2010}, while on the other hand our developed system works with a \emph{corpus independent} approach that directly sifts keywords from a single document without any previous or background information.

Regarding the automated ad creative generation process, to the best of our knowledge, this issue remains still an open problem in natural language processing and information retrieval areas as mentioned in\cite{DBLP:conf/ecir/Gabrilovich11}. Thus, the corresponding module of our system is an innovative contribution in this regard. 

%2. Adomaton Related
Assuming the ad auction mechanism of a search engine, the main issue that the advertisers are facing is to decide their bidding strategy and how they are going to split their budget among the keywords of their campaign. There have been various attempts to solve the budget optimization problem, some of which are based on heuristics, some calculate approximations using linear programming variations, and others take a more statistical and stochastic approach. Even Dar et al. \cite{EvenDar:2009} present their approach of maximizing profit, using a linear programming (LP) based polynomial-time algorithm. To deal with the NP-hardness of the problem, they propose a constant-factor approximation when the optimal profit significantly exceeds the cost. It is based on rounding a natural LP formulation of the problem. Szymanski and Lee \cite{Szymanski:2006} discuss how advertisers, by considering minimum return on investment (ROI), change their bidding and, consequently the auctioneer's revenue in sponsored search advertisement auctions. 

Borgs et al. \cite{borgsimmorlica2007} propose a bidding heuristic that is based on equalizing the marginal ROI across all keywords, so they change each keyword bid based on the ROI performance of the previous day. Their system converges to its market equilibrium in the case of the first price mechanism with a single slot when everybody adopts the proposed perturbed bid solution. 

Rusmevichientong and Williamson \cite{Rusmevichientong:2006} develop an adaptive algorithm that learns the proportions of clicks for different keywords by bidding on different prefix solutions, and eventually converges to near-optimal profits, assuming that various parameters are concentrated around their means. Muthukrishnan et al. \cite{Muthukrishnan:2010} consider stochastic algorithms that attempt to solve the problem in advance, and not by adaptive learning as in \cite{Rusmevichientong:2006}, and work for pre-specified probability distributions of keyword clicks. 

Zhou et al. \cite{Zhou:2008:BCB:1367497.1367747} model the problem of advertisers winning an ad slot for one keyword they bid upon as an online multiple-choice knapsack problem. Zhou and Naroditskiy \cite{Zhou:2008} continue the work of \cite{Zhou:2008:BCB:1367497.1367747} modeling budget-constrained keyword bidding as a stochastic multiple-choice knapsack problem. Their algorithm selects keywords based on a threshold function which can be built and updated using historical data. It employs distributional information about prices and tries to solve the bidding problem with multiple ad-position, keywords, and time periods.

The problem of finding a near-optimal bidding strategy has been also approached by using autonomous agents. The TAC Ad Auctions (TAC/AA) game investigates complex strategic issues found in real sponsored search auctions through a simulation of the general auction process \cite{springerlink:10.1007/978-3-642-15117-0_11}.

